Asymptotically Optimal Closed-Form Phase Configuration of $1$-bit RISs via Sign Alignment

While Reconfigurable Intelligent Surfaces (RISs) constitute one of the most prominent enablers for the upcoming sixth Generation (6G) of wireless networks, the design of efficient RIS phase profiles remains a notorious challenge when large numbers of phase-quantized unit cells are involved, typically of a single bit, as implemented by a vast majority of existing metasurface prototypes. In this paper, we focus on the RIS phase configuration problem for the exemplary case of the Signal-to-Noise Ratio (SNR) maximization for an RIS-enabled single-input single-output system where the metasurface tunable elements admit a phase difference of $\pi$ radians. We present a novel closed-form configuration which serves as a lower bound guaranteeing at least half the SNR of the ideal continuous (upper bound) SNR gain, and whose mean performance is shown to be asymptotically optimal. The proposed sign alignment configuration can be further used as initialization to standard discrete optimization algorithms. A discussion on the reduced complexity hardware benefits via the presented configuration is also included. Our numerical results demonstrate the efficacy of the proposed RIS sign alignment scheme over iterative approaches as well as the commonplace continuous phase quantization treatment.

==> acronyms.tex <==
% acronym

% \newacronym[plural=cMs,firstplural=centiMorgans (cMs)]{cM}{cM}{centiMorgan}

% \newacronym{tx}{Tx}{transmitter}

% \newacronym{rx}{Rx}{receiver}

% \newacronym{ris}{RIS}{reconfigurable intelligent surface}

% \newacronym{csi}{CSI}{channel state information}

% %\newacronym[plural=VUEs,firstplural=vehicular users (VUEs)]{vue}{VUE}{vehicular user}

% %\newacronym[plural=RSUs,firstplural=roadside units (RSUs)]{rsu}{RSU}{roadside unit}

% \newacronym{mle}{MLE}{maximum likelihood estimation}

% \newacronym{mmw}{mmWave}{millimeter wave}

% \newacronym{pl}{PL}{path loss}

% \newacronym{los}{LOS}{line-of-sight}

% \newacronym{nlos}{NLOS}{non line-of-sight}

% \newacronym{rss}{RSS}{received signal strength}

% \newacronym{pdf}{PDF}{probability distribution function}

% \newacronym{cdf}{CDF}{cummulative density function}

% \newacronym{gpr}{GPR}{Gaussian process regression}

% \newacronym{nn}{NN}{neural network}

% \newacronym{relu}{ReLU}{rectified linear unit}

% \newacronym{mlp}{MLP}{multi-layer perceptron}




\newacro{ANN}[ANN]{Artificial Neural Network}
\acrodefplural{ANN}[ANNs]{Artificial Neural Networks} 




\newacro{RIS}[RIS]{Reconfigurable Intelligent Surface}
\acrodefplural{RIS}[RISs]{Reconfigurable Intelligent Surfaces} 


\newacro{6G}[6G]{Sixth Generation}
\newacro{SNR}[SNR]{Signal-to-Noise Ratio}
\newacro{SINR}[SINR]{Signal-to-Interference-plus-Noise Ratio}
\newacro{TX}[TX]{Transmitter}

\newacro{RX}[RX]{Receiver}
\acrodefplural{RX}[RXs]{Receivers} 

\newacro{TVC}[TVC]{Time Varying Channel}
\acrodefplural{TVC}[TVCs]{Time Varying Channels}

\newacro{BS}[BS]{Base Station}
\newacro{UE}[UE]{User Equipment}
\acrodefplural{UE}[UEs]{Users Equipments}


\newacro{MSE}[MSE]{Mean Squared Error}

\newacro{MAC}[MAC]{Medium Access Control}

\newacro{NMSE}[NMSE]{Normalized Mean Squared Error}
\newacro{EM}[EM]{Electro-Magnetic}
\newacro{CSI}[CSI]{Channel State Information}
\newacro{MISO}[MISO]{Multiple-Input Single-Output}
\newacro{SISO}[MISO]{Single-Input Single-Output}
\newacro{NOMA}[NOMA]{Non-Orthogonal Multiple Access}
\newacro{OFDM}[OFDM]{Orthogonal Frequency-Division Multiplexing}
\newacro{QoS}[QoS]{Quality of Service}

\newacro{UAV}[UAV]{Unmanned Autonomous Vehicle}
\acrodefplural{UAV}[UAVs]{Unmanned Autonomous Vehicles}


\newacro{IoT}[IoT]{Internet of Things}
\newacro{LOS}[LOS]{Line Of Sight}
\newacro{NLOS}[NLOS]{Non-Line Of Sight}

\newacro{AoA}[AoA]{Angle of Arrival}
\acrodefplural{AoA}[AoAs]{Angles of Arrival}

\newacro{AoD}[AoD]{Angle of Departure}
\acrodefplural{AoD}[AoDs]{Angles of Departure}

\newacro{AWGN}[AWGN]{Additive White Gaussian Noise}
%\newacro{AI}[AI]{Artificial Intelligence}
%\newacro{ML}[ML]{Machine Learning}
%\newacro{DL}[DL]{Deep Learning}
\newacro{SL}[SL]{Supervised Learning}
\newacro{RL}[RL]{Reinforcement Learning}
\newacro{DRL}[DRL]{Deep Reinforcement Learning}

\newacro{MDP}[MDP]{Markov Decision Process}
\acrodefplural{MDP}[MDPs]{Markov Decision Processes} 

\newacro{POMDP}[POMDP]{Partially Observable Markov Decision Process}
\acrodefplural{POMDP}[POMDPs]{Partially Observable Markov Decision Processes} 


\newacro{DQN}[DQN]{Deep Q-Network}
\newacro{D$^3$QN}[D$^3$QN]{Duelling Double Deep Q Network}
\newacro{PG}[PG]{Policy Gradient}
\newacro{PPO}[PPO]{Proximal Policy Optimization}
\newacro{DDPG}[DDPG]{Deep Deterministic Policy Gradient}
\newacro{UCB}[UCB]{Upper Confidence Bound}
\newacro{GPU}[GPU]{Graphical Processing Unit}
\newacro{PDS}[PDS]{Post Decision State}
\newacro{TD}[TD]{Temporal Difference}
\newacro{MAML}[MAML]{Multi-Agent Reinforcement Learning}
\newacro{LSTM}[LSTM]{Long Short-Term Memory}
% \newacro{}[]{}


\newacro{EE}[EE]{Energy Efficiency}
\newacro{SE}[SE]{Spectral Efficiency}
\newacro{MIMO}[MIMO]{Multiple-Input Multiple-Output}

\newacro{IID}[IID]{Independent and Identically Distributed}


\newacro{MAB}[MAB]{Multi-Armed Bandits}
\newacro{CB}[CB]{Contextual Bandits}


%\newacro{DSP}[DSP]{Deep Softmax Prediction}
\newacro{DRP}[DRP]{Deep Reward Prediction}


\newacro{DFT}[DFT]{Discrete Fourier Transform}
\newacro{ML}[ML]{Machine Learning}


\newacro{SGD}[SGD]{Stochastic Gradient Descent}

\newacro{AI}[AI]{Artificial Intelligence}

==> old_text/Optimization_Procedures.tex <==
\section{Related $1$-bit Optimization Procedures}

The sign alignment procedure described in the previous section provides a minimal complexity approximate solution for $\mathcal{OP}_2$ with performance guarantees.
However, the aforedescribed methodology additionally allows for iterative optimization approaches to be developed, that are posed to provide higher SNR gains, albeit with increased computational requirements.
The approach presented in Section~\ref{sec:gradient-ascent} capitalizes on the modified objective $\mathcal{OP}_2$ to propose a continuous optimization approach with provable convergence,
while the algorithms of Sections~\ref{sec:hill-climbing},~\ref{sec:neuroevolution} utilize the obtained configuration of Algorithm~\ref{alg:1} as an initialization point.


\subsection{Gradient Ascent with Convergence at an Admissible Point}\label{sec:gradient-ascent}
For the current methodology, the discrete nature of $\mathcal{OP}_2$ is first transferred to the continuous domain via analytic continuation, as follows
\begin{align}\label{obj:analytic-continuation}
    \mathcal{OP}_3:~&~ \max \hat{\gamma}(\boldsymbol{\phi}) 
    \quad s.t.~ \boldsymbol{\phi} \in [-1, +1]^N.
\end{align}

\textcolor{red}{By examining the gradient properties of $\hat{\gamma}(\boldsymbol{\phi})$, it is $\partial \hat{\gamma}(\boldsymbol{\phi})/\partial \boldsymbol{\phi}_n = 2 \boldsymbol{a}_n \sum_{n=1}^{N} \boldsymbol{a}_n \boldsymbol{\phi}_n + 2 \boldsymbol{b}_n \sum_{n=1}^{N} \boldsymbol{b}_n \boldsymbol{\phi}_n$,
and similarly $\partial^2 \hat{\gamma}(\boldsymbol{\phi})/\partial^2 \boldsymbol{\phi}_n = 2 \boldsymbol{a}^2_n + 2 \boldsymbol{b}^2_n > 0$,
%Note that on statistical channel models (Rayleigh, Ricean), it is positive with probability 1.
Therefore, $\hat{\gamma}(\boldsymbol{\phi})$ is convex in $(-1, +1)^N$.
To search for its extrema, first notice that $\nabla \hat{\gamma}(\boldsymbol{\phi}) = \boldsymbol{0} \Leftrightarrow \boldsymbol{\phi} = \boldsymbol{0}$, which is a trivial solution.
Since $\hat{\gamma}$ is convex, that solution is a minima, and there is no other zero of the gradient function in $(-1, +1)^N$. Therefore, all maxima of $\hat{\gamma}$ reside on its boundaries, i.e. in $\{-1, +1\}^N$.
Thus, any maxima of $\hat{\gamma}$ is an admissible solution of $\gamma(\boldsymbol{\phi})$.}
Having said, that to arrive at one of the maxima, one can perform iterative gradient ascent updates so that the elements of the configuration vector are updated as $\myvec{\phi}^{k+1}_n \gets \myvec{\phi}^{k}_n + \alpha \partial \hat{\gamma}(\boldsymbol{\phi})/\partial \boldsymbol{\phi}_n$, during the $k$-th iteration for some step size $\alpha$ and initial starting point.
Since the ascent happens on the continuous landscape, it is expected for the algorithm to more efficiently progress into the search space, compared to large discrete jumps.

% The complete procedure is given in Algorithm~\ref{alg:2}.
% \begin{algorithm}
% \caption{Gradient ascent on $\mathcal{OP}_3$}\label{alg:2}
% \begin{algorithmic}[1]
% \Require CSI vector $\myvec{c}$, initial RIS profile $\myvec{\phi}^{0}$, step size $\alpha$
% \For{$k=0,\dots,$~\text{until convergence}}
%     \For{$n=1,\dots,N$}
%         \State $\myvec{\phi}^{k+1}_n \gets \myvec{\phi}^{k}_n + \alpha \frac{\partial \hat{\gamma}(\boldsymbol{\phi})}{\partial \boldsymbol{\phi}_n}$
%     \EndFor
% \EndFor
% \State \Return $\myvec{\phi}^{k}$
% \end{algorithmic}
% \end{algorithm}

% Since $\hat{\gamma}$ is convex, gradient ascent can be used to converge to one of the boundary points of $\hat{\gamma}$ which are known to be admissible solutions for the original problem.
% The motivation for using a gradient-based algorithm instead of searching directly solutions in the discrete cases is that the continuous landscape of the extended domain function is expected to guide the gradient steps toward a better discrete solution that those of discrete programming -- which disregards information in-between the vertices of the discrete hypercube.


\subsection{Hill Climbing}\label{sec:hill-climbing}
Since $\mathcal{OP}_2$ is a discrete optimization problem, one of the typical baseline approaches is to start with a random candidate solution, loop through its elements, attempt to flip its value from $\phi^{0}$ to $\phi^{\pi}$ and vice-versa, evaluate the objective function after the flip is performed, and discard the change if no gain was obtained. 
This procedure, termed ``coordinate hill climbing'', is described in Algorithm~\ref{alg:3}.
In this work, we propose to select $\myvec{\phi}^{S.A.}$ of Algorithm~\ref{alg:1} as a starting configuration.
This has the two-fold benefit of starting the search from an already improved point, compared to random initialization, and higher performance guarantees:
Since the hill climbing algorithm can only improve on any given configuration, the performance bounds of Section~\ref{sec:sign-alignment-analysis} hold for Algorithm~\ref{alg:3} as well. 
\begin{algorithm}
\caption{Coordinate hill climbing on $\mathcal{OP}_2$}\label{alg:3}
\begin{algorithmic}[1]
\Require CSI vector $\myvec{c}$
\State  $\myvec{\phi}^0 \gets \myvec{\phi}^{S.A.}$ from Algorithm~\ref{alg:1}
\State $\gamma^{\rm max} \gets \gamma(\myvec{\phi}^0)$
\State $k \gets 1$
\While{$k>1$ AND $\myvec{\phi}^{k-1} \neq \myvec{\phi}^{k-2}$}
    \For{$n=1,\dots,N$}
        \State $\myvec{\phi}^{k}_n \gets - \myvec{\phi}^{k-1}_n$
    
        \If {$\gamma(\myvec{\phi}^{k}) > \gamma^{\rm max}$}
            \State $\gamma^{\rm max} \gets \gamma(\myvec{\phi}^{k})$
        \Else
            \State $\myvec{\phi}^{k}_n \gets \myvec{\phi}^{k-1}_n$
        \EndIf
    \EndFor
    \State $k \gets k + 1$
\EndWhile
\State \Return $\myvec{\phi}^{k}$
\end{algorithmic}
\end{algorithm}



\subsection{Kernel-based Evolution Strategies}\label{sec:neuroevolution}
Another popular approach for optimizing RISs with discrete phase shifts is Genetic Optimization (GO), since it is a black box algorithm that works particularly well when the discrete optimized vector can be meaningfully expressed as a string of bits.
Nevertheless, the application of GO in RIS optimization with large numbers of unit elements does not always lead to desired performance.
The is explained for one part, since the pseudo-random search in the discrete domain is much less efficient than optimization step on continuous landscapes, but the suboptimal performance can also be attributed to the fact that ``off-the-shelf'' GO algorithms are not design to take account correlations among the desired phases of nearby unit elements within the surface.

In fact, when even moderately LoS-dominated channel conditions are applicable, the optimal phase configurations of RISs exhibit strong spatial positive or negative correlations among its elements. 
Motivated by the above, we propose a novel GO algorithm that uses local neighborhood information to determine the phase shift of each RIS element.
This approach takes inspiration from convolutional neural networks in deep learning as well as neural evolution strategies from reinforcement learning and aims to optimize the continuous parameters of a 2D kernel, which is then applied via standard 2D convolution onto neighborhoods of unit elements over the RIS surface, given an existing configuration.

Precisely, let us define a convolutional kernel matrix $\boldsymbol{W} \in \mathbb{R}^{K\times K}$, where $K$ is an odd positive number specifying the size of the kernel.
In the following, we assume that $N$ is a perfect square and that the RIS elements are placed on a $(\sqrt{N} \times \sqrt{N})$ planar array, so that $\boldsymbol{\phi}_{k,l}$ denotes the element of the $k$-th columns and $l$-th row.
Then, given an existing configuration $\boldsymbol{\phi}$, the phase of the unit cell is updated as follows
\begin{equation}\label{eq:conv-update}
    \boldsymbol{\phi}_{k,l} = {\rm conv}_{k,l}(\boldsymbol{\phi}, \boldsymbol{W}) \triangleq \sum_{i=k-\frac{(K-1)}{2}}^{k+\frac{(K-1)}{2}} ~ \sum_{j=l-\frac{(K-1)}{2}}^{l+\frac{(K-1)}{2}} \boldsymbol{W}_{i,j} \boldsymbol{\phi}_{i,j},
\end{equation}
where the out-of-bounds cells are arbitrarily treated as zeros.
Note that applying~\eqref{eq:conv-update} over all $\boldsymbol{\phi}_{k,l}$ once, only provides updates based from its neighboring units. To let the information flow more efficiently to the complete surface, we chose to apply~\eqref{eq:conv-update} on all pixels $T$ consecutive times in sequence.
To bootstrap this procedure, we start each sequence having the initial configuration $\myvec{\phi}^{S.A.}$ of Algorithm~\ref{alg:1}, since this configuration is expected to have already captured some spatial correlations.
To ensure the final $\myvec{\phi}$ values belong in $\mathcal{F}$, the ${\rm sign()}$ function is applied to the resulting phase configuration after the $T$-th iteration, as shown in Algorithm~\ref{alg:phi-update-kernel}

\begin{algorithm}
\caption{Kernel-based update of RIS configuration}\label{alg:phi-update-kernel}
\begin{algorithmic}[1]
\Require Existing RIS configuration $\myvec{\phi}$, kernel $\boldsymbol{W}$
\State $\myvec{\phi}^{0} \gets \myvec{\phi}$
\For {$t=1,\dots,T$}
        \For{$k=1,\dots,\sqrt{N}$}
            \For{$l=1,\dots,\sqrt{N}$}
                \State $\myvec{\phi}_{k,l}^{t} \gets {\rm conv}_{k,l}(\boldsymbol{\phi}^{t-1}, \boldsymbol{W})$
            \EndFor
        \EndFor
\EndFor
\State $\boldsymbol{\phi}^{\rm E.S.} \gets {\rm sign}(\boldsymbol{\phi}^{t})$
\State \Return $\boldsymbol{\phi}^{\rm E.S.}$
\end{algorithmic}
\end{algorithm}




It is highlighted that the aforementioned parametric update rule has $K^2$ parameters, which are intended to be orders of magnitude fewer than the $N$ elements of the RIS and grow assyptotically slower, as it is typical when using convolutional kernels in image processing.
Furthermore, despite $\myvec{\phi}$ being a discrete vector, the parameters of $\boldsymbol{W}$ that require optimization are themselves continuous.
Therefore, the resulting optimization procedure can be more efficiently tackled via GO algorithms.
In this work, we use Evolution Strategies (ES) as our genetic optimizer.
The overall algorithm is given in Algorithm~\ref{alg:ES}

\begin{algorithm}
\caption{Kernel-based evolution strategies for RIS tuning}\label{alg:ES}
\begin{algorithmic}[1]
\Require CSI vector $\myvec{c}$, population size $P$, noise standard deviation $\tilde{sigma}$, step size $\alpha$, initial kernel parameters $\boldsymbol{W}^0$ 
\State  Compute $\myvec{\phi}^{S.A.}$ from Algorithm~\ref{alg:1}
\For{$t'=1,\dots,$~until convergence}
    \State Sample $\epsilon^1,\dots,\epsilon^p \sim \mathcal{N}(0, \tilde{\sigma}\boldsymbol{I})$
    \State Compute $\myvec{\phi}^{p}$ from Algorithm~\ref{alg:phi-update-kernel} using $\myvec{\phi}^{S.A.}$ and $\boldsymbol{W}^{t'-1}+\epsilon^p$ for $p=1,\dots,P$
    \State Compute $\gamma^p(\myvec{\phi}^{p})$ from $\mathcal{OP}_2$ for $p=1,\dots,P$
    \State $\boldsymbol{W}^{t'} \gets \frac{\alpha}{P\tilde{\sigma}}\sum_{p=1}^{P} \epsilon^p \gamma^p(\myvec{\phi}^{p})$ 
\EndFor
\State Compute final $\boldsymbol{\phi}^{\rm E.S.}$ from Algorithm~\ref{alg:phi-update-kernel} using $\myvec{\phi}^{S.A.}$ and $\boldsymbol{W}^{t'}$
\State \Return $\myvec{\phi}^{S.A.}$. 
\end{algorithmic}
\end{algorithm}



==> old_text/results_dirty.tex <==
\section{Results (DIRTY)}


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/SNR_VS_N_w_ricean_factor6_w_errorbars.png}
    \caption{SNR over N for Ricean factor of 6dB}
    \label{fig:sns-vs-N-6-dB}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/SNR_VS_N_w_ricean_factor20_w_errorbars.png}
    \caption{SNR over N for Ricean factor of 20dB}
    \label{fig:sns-vs-N-20-dB}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/SNR_VS_Ricean_factor_N_256_w_errorbars.png}
    \caption{SNR over Ricean factor (in dB) for a RIS with 256 elements.}
    \label{fig:sns-vs-ricean-1}
\end{figure}

